Evolution of statistical analysis in empirical software engineering research: Current state and steps forward

Software engineering research is evolving and papers are increasingly based on empirical data from a multitude of sources, using statistical tests to determine if and to what degree empirical evidence supports their hypotheses. To investigate the practices and trends of statistical analysis in empirical software engineering (ESE), this paper presents a review of a large pool of papers from top-ranked software engineering journals. First, we manually reviewed 161 papers and in the second phase of our method, we conducted a more extensive semi-automatic classification of papers spanning the years 2001--2015 and 5,196 papers. Results from both review steps was used to: i) identify and analyze the predominant practices in ESE (e.g., using t-test or ANOVA), as well as relevant trends in usage of specific statistical methods (e.g., nonparametric tests and effect size measures) and, ii) develop a conceptual model for a statistical analysis workflow with suggestions on how to apply different statistical methods as well as guidelines to avoid pitfalls. Lastly, we confirm existing claims that current ESE practices lack a standard to report practical significance of results. We illustrate how practical significance can be discussed in terms of both the statistical analysis and in the practitioner's context.

==> sections/06pracsign.tex <==
As we previously showed, \textless 50\% of the manually classified publications explicitly discussed practical significance. The semi-automatic classification provided the same indications, see Figure~\ref{fig:combined}. (`Practical significance'), although this is one of the harder analyzes for the tool to make. 

To be clear, we believe it would help the software engineering community if researchers are: $i$) Expected to explicitly report on practical significance in their studies (when appropriate), $ii$) not allowed to make implicit arguments for practical significance based solely on the nature of the problem\slash context, e.g., ``Company $A$ thought this was important'' and, $iii$) required to clearly connect any findings with own or others' evidence that support them. The evidence should be grounded in a mature statistical analyzes, possibly based on the \texttt{SMM}.

We argue that an analysis of practical significance should ideally consider:

\begin{enumerate}
    \item \textbf{Contexts.} Identify the practical contexts in which the found effect is important. The context typically includes which type of domain, company\slash organization type, size, experience level etc. See \citet{petersenW2009context} for a detailed model of contexts.

    \item \textbf{Affected variables.} Identify which variables would be affected by the effect in the affected contexts. Variables are typically high-level observables like cost, effort\slash time, or quality, but can also be more detailed metrics related to the top-level ones.

    \item \textbf{Absolute practical significance.} Argue for why the size of the effect shown by the statistical analysis would have practical significance for the identified variables in the given contexts. The maturity of this argument is based on what type of evidence is given:
    
    \begin{enumerate}
        \item \textbf{Reason-from-common-sense.} Researchers assume it is evident to the reader once the effect has been stated or refers to grey literature opinions about relevant levels.

        \item \textbf{Comparison-to-published-literature.} Compares effects to relevant variable levels as supported by empirical data in published literature

        \item \textbf{Static-interpretation.} Have asked practitioners in the relevant contexts and presents evidence of their interpretations of how important the effect of the identified size would be.

        \item \textbf{Dynamic-interpretation.} Have asked practitioners in the relevant contexts and presents evidence of their interpretations of how important the effect of the identified size seen in their context actually is for them.
    \end{enumerate}

    \item \textbf{Relative practical significance.} Argue for how the effect seen fares in relation to alternative methods of changing the affected variables. The argument here can be at the same a-d refinement levels used in \#3 above.

\end{enumerate}

We argue that the absolute practical significance (Item 3) does not make sense and cannot fully be described if one has not identified the variables in Item 2. And they in turn depend on the context identified in Item 1. Although an explicit discussion of the (absolute) practical significance in Item 3 can often be considered enough there are always alternative solutions that can be selected. The analysis in Item 4 aims at clearly discussing how the established effects Item 3's significance relates to existing, published or in use in an industrial\slash practical context, solutions.

For reasons of brevity we do not detail the model further here but leave applications, evaluation and refinement to future work.

